Efficiently Bounding Optimal Solutions after Small Data Modification in Large-Scale Empirical Risk Minimization

We study large-scale classification problems in changing environments where a small part of the dataset is modified, and the effect of the data modification must be quickly incorporated into the classifier. When the entire dataset is large, even if the amount of the data modification is fairly small, the computational cost of re-training the classifier would be prohibitively large. In this paper, we propose a novel method for efficiently incorporating such a data modification effect into the classifier without actually re-training it. The proposed method provides bounds on the unknown optimal classifier with the cost only proportional to the size of the data modification. We demonstrate through numerical experiments that the proposed method provides sufficiently tight bounds with negligible computational costs, especially when a small part of the dataset is modified in a large-scale classification problem.

==> appC.tex <==
\section{Detailed experimental results} \label{app:exp}

\begin{table}[b]
\begin{center}
\begin{minipage}[c]{0.45\hsize}
\caption{Data sets used for the experiment}
\label{table:datasets}
\begin{itemize}
\item All are from LIBSVM data repository \cite{chang2011libsvm}.
\item 80\% of instances are used for training while others are for validation.
\item Every instance $\bm{x}$ is normalized to norm $\|\bm{x}\|_2 = 1$.
\end{itemize}
\end{minipage}
\begin{minipage}[c]{0.45\hsize}
\begin{tabular}{crr}
\hline
Name & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{$d$} \\
\hline
{\tt kdd-a}      & 8,407,752 & 20,216,830 \\
{\tt url}        & 2,396,130 &  3,231,961 \\
{\tt news20}     &    19,996 &  1,355,191 \\
{\tt real-sim}   &    72,309 &     20,958 \\
{\tt rcv1-train} &    20,242 &     47,236 \\
\hline
\end{tabular}
\end{minipage}
\end{center}
\end{table}

In this section we show the whole experimental results. We conducted experiments for the five data sets in Table \ref{table:datasets} and $\lambda \in \{0.001, 0.01, 0.1, 1\}$.

Figures \ref{fig:experiment-all-1} to \ref{fig:experiment-all-4} show the results of the label determination rate,
%for $\lambda = \{0.001, 0.01, 0.1, 1\}$,
Figures \ref{fig:experiment-all-5} to \ref{fig:experiment-all-8} show the upper bound of the parameter change,
and Table \ref{table:computation-time-all} show the ratio of the computation time of bound computation in \S\ref{sec:main} to re-training.

%in Tables \ref{fig:experiment-all-1} to \ref{fig:experiment-all-8}.

\input{experiment-table-all}

\begin{table}[tp]
\caption{The ratio of the computation time of the bound computation to re-training (with warm-start)}
\label{table:computation-time-all}
\begin{center}
{\tiny
\begin{tabular}{c|rrr|rrr|rrr}
\hline
& \multicolumn{3}{c|}{(a) spot modification} & \multicolumn{3}{c|}{(b) instance modification} & \multicolumn{3}{c}{(c) feature modification} \\
 & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{100} & \multicolumn{1}{c|}{10000}
 & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c|}{100}
 & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{100} \\
\hline
\multicolumn{10}{c}{$\lambda = 01$} \\
\hline
{\tt kdd-a} & $3\times 10^{-6}$ & $1\times 10^{-4}$ & $1\times 10^{-4}$ & $5\times 10^{-7}$ & $2\times 10^{-4}$ & $1\times 10^{-2}$ & $2\times 10^{-7}$ & $5\times 10^{-7}$ & $5\times 10^{-5}$ \\
{\tt url} & $5\times 10^{-8}$ & $2\times 10^{-5}$ & $5\times 10^{-5}$ & $3\times 10^{-7}$ & $2\times 10^{-3}$ & $3\times 10^{-2}$ & $3\times 10^{-5}$ & $3\times 10^{-6}$ & $4\times 10^{-5}$ \\
{\tt news20} & $2\times 10^{-6}$ & $3\times 10^{-5}$ & $5\times 10^{-3}$ & $7\times 10^{-5}$ & $2\times 10^{-3}$ & $6\times 10^{-2}$ & $4\times 10^{-6}$ & $1\times 10^{-5}$ & $4\times 10^{-4}$ \\
{\tt real-sim} & $9\times 10^{-6}$ & $1\times 10^{-4}$ & $7\times 10^{-3}$ & $5\times 10^{-5}$ & $4\times 10^{-4}$ & $2\times 10^{-3}$ & $1\times 10^{-4}$ & $6\times 10^{-4}$ & $2\times 10^{-3}$ \\
{\tt rcv1-train} & $2\times 10^{-5}$ & $2\times 10^{-4}$ & $1\times 10^{-2}$ & $2\times 10^{-4}$ & $5\times 10^{-4}$ & $6\times 10^{-3}$ & $5\times 10^{-5}$ & $2\times 10^{-4}$ & $2\times 10^{-3}$ \\
\hline
\multicolumn{10}{c}{$\lambda = 0$} \\
\hline
{\tt kdd-a} & $6\times 10^{-6}$ & $3\times 10^{-6}$ & $2\times 10^{-4}$ & $1\times 10^{-6}$ & $1\times 10^{-4}$ & $1\times 10^{-2}$ & $5\times 10^{-7}$ & $1\times 10^{-6}$ & $2\times 10^{-4}$ \\
{\tt url} & $1\times 10^{-7}$ & $3\times 10^{-6}$ & $8\times 10^{-5}$ & $6\times 10^{-6}$ & $3\times 10^{-3}$ & $5\times 10^{-2}$ & $9\times 10^{-8}$ & $1\times 10^{-6}$ & $3\times 10^{-5}$ \\
{\tt news20} & $3\times 10^{-6}$ & $6\times 10^{-5}$ & $7\times 10^{-3}$ & $8\times 10^{-4}$ & $3\times 10^{-3}$ & $5\times 10^{-2}$ & $1\times 10^{-5}$ & $4\times 10^{-5}$ & $7\times 10^{-4}$ \\
{\tt real-sim} & $1\times 10^{-5}$ & $2\times 10^{-4}$ & $9\times 10^{-3}$ & $7\times 10^{-5}$ & $4\times 10^{-4}$ & $3\times 10^{-3}$ & $2\times 10^{-4}$ & $1\times 10^{-3}$ & $4\times 10^{-3}$ \\
{\tt rcv1-train} & $2\times 10^{-5}$ & $3\times 10^{-4}$ & $2\times 10^{-2}$ & $2\times 10^{-4}$ & $1\times 10^{-3}$ & $9\times 10^{-3}$ & $8\times 10^{-5}$ & $4\times 10^{-4}$ & $2\times 10^{-3}$ \\
\hline
\multicolumn{10}{c}{$\lambda = 0.1$} \\
\hline
{\tt kdd-a} & $2\times 10^{-7}$ & $4\times 10^{-6}$ & $1\times 10^{-4}$ & $4\times 10^{-7}$ & $5\times 10^{-6}$ & $2\times 10^{-2}$ & $2\times 10^{-7}$ & $2\times 10^{-6}$ & $1\times 10^{-5}$ \\
{\tt url} & $1\times 10^{-7}$ & $2\times 10^{-6}$ & $8\times 10^{-5}$ & $4\times 10^{-7}$ & $4\times 10^{-4}$ & $5\times 10^{-2}$ & $2\times 10^{-7}$ & $1\times 10^{-6}$ & $5\times 10^{-5}$ \\
{\tt news20} & $4\times 10^{-6}$ & $4\times 10^{-5}$ & $8\times 10^{-3}$ & $6\times 10^{-5}$ & $3\times 10^{-3}$ & $1\times 10^{-2}$ & $6\times 10^{-6}$ & $3\times 10^{-5}$ & $7\times 10^{-4}$ \\
{\tt real-sim} & $1\times 10^{-5}$ & $2\times 10^{-4}$ & $2\times 10^{-2}$ & $8\times 10^{-5}$ & $5\times 10^{-4}$ & $5\times 10^{-3}$ & $2\times 10^{-4}$ & $1\times 10^{-3}$ & $6\times 10^{-3}$ \\
{\tt rcv1-train} & $3\times 10^{-5}$ & $4\times 10^{-4}$ & $2\times 10^{-2}$ & $3\times 10^{-4}$ & $2\times 10^{-3}$ & $9\times 10^{-3}$ & $9\times 10^{-5}$ & $5\times 10^{-4}$ & $1\times 10^{-3}$ \\
\hline
\multicolumn{10}{c}{$\lambda = 1$} \\
\hline
{\tt kdd-a} & $3\times 10^{-7}$ & $3\times 10^{-6}$ & $2\times 10^{-4}$ & $5\times 10^{-7}$ & $6\times 10^{-6}$ & $2\times 10^{-2}$ & $2\times 10^{-7}$ & $2\times 10^{-6}$ & $2\times 10^{-5}$ \\
{\tt url} & $1\times 10^{-7}$ & $2\times 10^{-6}$ & $3\times 10^{-4}$ & $5\times 10^{-7}$ & $8\times 10^{-3}$ & $5\times 10^{-2}$ & $2\times 10^{-7}$ & $2\times 10^{-6}$ & $7\times 10^{-5}$ \\
{\tt news20} & $4\times 10^{-6}$ & $1\times 10^{-4}$ & $6\times 10^{-3}$ & $2\times 10^{-4}$ & $2\times 10^{-3}$ & $9\times 10^{-3}$ & $6\times 10^{-6}$ & $2\times 10^{-5}$ & $1\times 10^{-3}$ \\
{\tt real-sim} & $3\times 10^{-5}$ & $2\times 10^{-4}$ & $1\times 10^{-2}$ & $1\times 10^{-4}$ & $5\times 10^{-4}$ & $5\times 10^{-3}$ & $2\times 10^{-4}$ & $2\times 10^{-3}$ & $8\times 10^{-3}$ \\
{\tt rcv1-train} & $5\times 10^{-5}$ & $4\times 10^{-4}$ & $2\times 10^{-2}$ & $3\times 10^{-4}$ & $2\times 10^{-3}$ & $2\times 10^{-2}$ & $2\times 10^{-4}$ & $4\times 10^{-4}$ & $4\times 10^{-3}$ \\
\hline
\end{tabular}
}
\end{center}
\end{table}


==> appD.tex <==
Finally, let us discuss the connection with safe screening \cite{xxx}. 
%
In the example of smoothed hinge SVM (see \eqref{eq:smoothed-hinge1} and \eqref{eq:smoothed-hinge2}),
the optimality condition indicates that 
\begin{subequations} %15:26'ÌŽ®ŒQ
 \label{eq:smoothed-hinge-opt-cond} 
  \begin{align}
   \label{eq:smoothed-hinge-opt-cond.a} 
   y_i \bm x_i^\top \tilde{\bm {w}}^* < 1 - \gamma
   &~\Rightarrow~
   \tilde{\alpha}^*_i = 1,
   \\
   \label{eq:smoothed-hinge-opt-cond.b} 
   y_i \bm x_i^\top \tilde{\bm {w}}^* \in [1 - \gamma, 1]
   &~\Rightarrow~
   \tilde{\alpha}^*_i \in [0, 1], 
   \\
   \label{eq:smoothed-hinge-opt-cond.c} 
   1 < y_i \bm x_i^\top \tilde{\bm {w}}^*
   &~\Rightarrow~
   \tilde{\alpha}^*_i = 0.
  \end{align}
\end{subequations}
%
The third optimality condition indicates that
$L(y_i \bm x_i^\top \tilde{\bm {w}}^*) > 1 ~\Rightarrow~ \tilde{\alpha}^*_i = 0$,a
which means that the $i^{\rm \th}$ instance would be non-SV, and we can exclude the instance in the optimization,
which is reffered to as \emph{safe sample screening}\cite{ogawa2013safe,wang2013scaling,Zimmert2015}\footnote{
When training a smoothed-hinge SVM,
it is beneficial to know which of 
\eqref{eq:smoothed-hinge-opt-cond.a}, \eqref{eq:smoothed-hinge-opt-cond.b} or \eqref{eq:smoothed-hinge-opt-cond.c}
each instance is categorized into.
%
Using the bounds, even if the optimal solution
($\tilde{\bm {w}}^*$, $\tilde{\bm \alpha}^*$)
is not available, 
we can tell 
\begin{align*}
 U(y_i \bm x_i^\top \tilde{\bm {w}}^*) < 1 - \gamma
 &~\Rightarrow~ 
 \eqref{eq:smoothed-hinge-opt-cond.a} 
 \\
 (L(\tilde{\alpha}^*_i) > 0 \cap U(\tilde{\alpha}^*_i)) < 1
 \cup
 (L(y_i \bm x_i^\top \tilde{\bm {w}}^*) \ge 1 - \gamma \cap U(y_i \bm x_i^\top \tilde{\bm {w}}^*) \le 1)
 &~\Rightarrow~
 \eqref{eq:smoothed-hinge-opt-cond.b} 
 \\
 L(y_i \bm x_i^\top \tilde{\bm {w}}^*) 
 &~\Rightarrow~ 
 \eqref{eq:smoothed-hinge-opt-cond.c} 
\end{align*}
}.


